Quantum many-body scars as remnants of stable many-body periodic orbits

Quantum many-body scars (QMBS) represent a weak ergodicity-breaking phenomenon that defies the common scenario of thermalization in closed quantum systems. They are often regarded as a many-body analog of quantum scars (QS) -- a single-particle phenomenon in quantum chaos -- due to their superficial similarities. However, unlike QS, a clear connection between QMBS and classical chaos has remained elusive. It has nevertheless been speculated that in an appropriate semiclassical limit, QMBS should have a correspondence to weakly unstable periodic orbits. In this paper, I present a counterexample to this conjecture by studying a bosonic model with a large number of flavors. The dynamics of out-of-time-ordered correlators (OTOCs) suggest that QMBS do not display chaotic behavior in the semiclassical limit. In contrast, chaotic dynamics are expected for initial states not associated with QMBS. Interestingly, the anomalous OTOC dynamics persist even under weak perturbations that eliminate the scarred eigenstates, suggesting a certain robustness in the phenomenon.

==> perturbation.tex <==
%\textit{Perturbations.}--It is known that certain types of perturbations can stabilize the oscillations starting from the N\'eel state. We focus on perturbations discussed in Ref.~\cite{nearly_su2} and in Ref.~\cite{Kieran2020}, and show that our approximate wave function $\ket{S_n}$ becomes even better approximation. In this section, we denote the scar states of perturbed PXP model by $\ket*{\mc{S}_n}$ and their energy by $E_n$. We numerically find that squared overlap $|\innerproduct*{S_n}{\mc{S}_n}|^2>0.95$ for $N=10$ when perturbations in Ref.~\cite{nearly_su2} and in Ref.~\cite{Kieran2020} are added. Particularly with perturbations $\delta H$ from Ref.~\cite{Kieran2020}, $E_n$ is quite close to $n\sqrt{2}$, which implies that $\delta H$ almost satisfies the following relation: for $\forall n$,
%\begin{equation}
    %A\begin{split}
        %P_{\mr{Ryd}}\left(H_{\mr{anil}1}+\delta H\right)\ket*{\wtil{S}_n}=0.
    %\end{split}
%\end{equation}

%We consider the following ``first-order" correction which is included in both sets of perturbations in Ref.~\cite{nearly_su2} and Ref.~\cite{Kieran2020}:
%\begin{equation}\label{eq:DH}
%\Delta H(\lambda)\coloneqq\lambda\sum_{i\in\Lambda}P_{i-1}X_iP_{i+1}(P_{i-2}+P_{i+2}),
%\end{equation}
%where $\lambda$ is a coefficient. As shown in Fig.~[FIG], when $\lambda=0.11$ which is close to ones obtained in Ref.~\cite{nearly_su2, Kieran2020}, $\Delta H(\lambda)$ already makes the scar states $\ket*{\mc{S}_n}$ almost equidistant and $|\innerproduct*{\mc{S}_n}{S_n}|^2>0.95$. We will rationalize this value in the following. In the spin-$1$ basis, we find that $P_{\mr{Ryd}}\left(H_{\mr{anil}1}+\Delta H(\lambda)\right)\ket*{\wtil{S}_n}=P_{\mr{Ryd}}H_{\mr{rem}}(\lambda)\ket*{\wtil{S}_n}$, where% relevant terms in $H_{\mr{anil}1}+\Delta H(\lambda)$, i.e., terms that do not annihilate $\ket*{\wtil{S}_n}$ are written as $\sum_{b\in\Lambda_{\mr{B}}}h_b(\lambda)$, where 
%\begin{widetext}
%\begin{equation}
    %\begin{split}
        %H_{\mr{rem}}(\lambda)\coloneqq\sum_{b\in\Lambda_{\mr{B}}}&\Bigg[\frac{-1+\lambda}{\sqrt{6}}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{T_{2,0}}_{b,b+1}+\frac{\lambda}{2}\left(\left(\ket*{0,0}-\ket*{+,+}\right)\bra*{T_{2,1}}_{b,b+1}+\left(\ket*{0,0}-\ket*{-,-}\right)\bra*{T_{2,-1}}_{b,b+1}\right)\\
        %&-\lambda\left(\dyad*{+,0,+}{T_{3,3}}+\dyad*{-,0,-}{T_{3,-3}}\right)_{b,b+1,b+2}-\frac{\lambda}{3}\left(\dyad*{+,0,0}{T_{3,2}}+\dyad*{0,0,-}{T_{3,-2}}\right)_{b,b+1,b+2}\Bigg].
    %\end{split}
%\end{equation}
%\end{widetext}
%We also define the two-body terms as $h_b^2(\lambda)$ and the three-body terms as $h_b^3(\lambda)$. 
%One can roughly estimate an optimal $\lambda$ that makes $h_b(\lambda)$ most negligible. As $\mr{Tr}\left(h_b(\lambda)\right)^\dag h_b(\lambda)$ is smallest at $\lambda=3\sqrt{6}/(32\sqrt{6}-3)\cong0.09748$, we expect that at around this value the perturbation $\Delta H(\lambda)$ is most effective, and this roughly agrees with the numerical value. 
%We numerically observe that $\sum_{n=1}^N\norm*{P_{\mr{Ryd}}H_{\mr{rem}}(\lambda)\ket*{\wtil{S}_n}}^2$ becomes smallest at $\lambda\cong0.1168$ for $N=10$, which agrees with both our estimate above and the other numerical values. 
\label{sec:perturbation}
Certain modifications of the PXP Hamiltonian, $H\to H+\delta H$, have been known to stabilize the long-lived  oscillations in dynamics starting from the N\'eel state, {particularly in the 1D chain}; e.g. perturbations of the form $\delta H_d=\lambda_d\sum_{i\in\Lambda_{\mr{B}}}P_{i-1}X_iP_{i+1}(Z_{i-d}+Z_{i+d})$ with $Z\coloneqq\dyad*{\uparrow}-\dyad*{\downarrow}$ and $2\leq d\leq N$ in Ref.~\cite{nearly_su2}, or terms generated by the commutation of parts of the Hamiltonian, which are regarded as ladder operators in an $SU(2)$ algebra, cf.~Ref.~\cite{Kieran2020}.
Below we will use the same notations for the exact scar states as for those of the unperturbed Hamiltonian.
%\begin{figure}
    %\centering
    %\includegraphics[width=0.48\textwidth]{overlap_FPs_pert.pdf}
    %\caption{\MM{Why don't you show all overlaps in one single figure, combining Fig 1+2?} Square of the overlap  $|\innerproduct*{\mc{S}_n^{\mr{PXP}}}{S_n}|^2$ between the exact scar states from numerics and the approximate wave function Eq.~(\ref{3}), for $N=10$ block spins. Blue dots, or ``emergent $SU(2)$" correspond to the perturbations discussed in Ref.~\cite{nearly_su2} and orange dots, or $\delta H$ correspond to the perturbation in Ref.~\cite{Kieran2020}.}
    %\label{fig:overlap_FPs}
%\end{figure}
%\begin{figure}
    %\centering
    %\includegraphics[width=0.48\textwidth]{energy_liealg.pdf}
    %\caption{\MM{I am not sure this should take so much space. It could be an inset to the overlap figure maybe?} Spectrum $\{E_n\}$ of the scar states $\ket*{\mc{S}_n^{\mr{PXP}}}$ in the scar-enhanced PXP model $H+\delta H$.}
    %\label{fig:energy_liealg}
%\end{figure}
Upon adding the scar-enhancing perturbation $\delta H_{\mr{SU}(2)}$ from Ref.~\cite{nearly_su2} or $\delta H_{\mr{Lie}}$ from Ref.~\cite{Kieran2020} to the PXP Hamiltonian  of a  1D chain, we numerically found very high overlaps $|\innerproduct*{S_n}{\mc{S}^{\mr{PXP}}_n}|^2>0.95$ with our trial states in chains of $N_b=10$ blocks, cf. Fig.~\ref{fig:<Sn|Sn> squared}. 
Moreover, for $\delta H_{\mr{Lie}}$ we found $E_n$ to approach the eigenvalues of $H_Z$, namely $n\sqrt{2}$, up to tiny deviations of order $\order{10^{-3}}$ (see the insert in Fig.~\ref{fig:<Sn|Sn> squared}). In contrast, the trial wavefunctions based on MPS, $\ket*{\mr{MPS}_n}$, become less and less accurate approximations (the squared overlap $|\innerproduct*{\mc{S}_n^{\mr{PXP}}}{\mr{MPS}_n}|^2$ drops to less than $40\%$ , see Fig.~\ref{fig:overlap_MPs}). 

A very high overlap and equidistant energies of $H+\delta H_{\mr{Lie}}$ imply that
\begin{equation}\label{eq:(H+dH)|S>}
\nonumber
    \begin{split}
        (H+\delta H_{\mr{Lie}})\ket*{S_n}&=P_{\mr{Ryd}}\left(H_{\mr{Z}}+H_1+H_2+\delta H_{\mr{Lie}}\right)\ket*{\wtil{S}_{n}}\\
        &
        \approx n\sqrt{2}\ket*{S_n},
    \end{split}
\end{equation}
which in turn reveals the important property that $P_{\mr{Ryd}}\left(H+\delta H_{\mr{Lie}}-H_{\mr{Z}}\right)\ket*{\wtil{S}_n} \equiv P_{\mr{Ryd}}H_{\rm ann}'\ket*{\wtil{S}_n}\approx 0$, where
we have defined
\begin{equation}
H_{\rm ann}' = H_1+H_2+\delta H_{\mr{Lie}}.
\end{equation}
%Eq.~\eqref{eq:(H+dH)|S>} implies that $P_{\mr{Ryd}}\left(H_1+H_2+\delta H\right)\ket*{\wtil{S}_n}\cong 0$. 
%Note that this relation reduces to $P_{\mr{Ryd}}(H_1+\delta H)\ket*{\wtil{S}_n}\cong0$ as $P_{\mr{Ryd}}H_2=0$. 
%{\em Here or a bit later we need to say sth like:} 
The above suggests that the PXP models {on the 1D chain} with improved scar properties were inadvertedly such that their scar space approached the Rydberg projected maximal spin space spanned by the trial states of Eq.~(\ref{eq:trial state}). This in turn implies that the dynamics starting from the N\'eel state is the projection on ${\cal V}_{\mr{Ryd}}$ of a simple precession {of a spin-coherent state} described by the Zeeman term $H_{\mr{Z}}$ in the effective pseudospin $S=1$ space of block spins, cf. Fig.~\ref{fig:illustration}. %\MM{check that we don't repeat this statement.}

The above structure suggests how the PXP model fits into the universal framework of QMBS outlaid in \blue{Sec.~\ref{sec:phenomenology}}, provided we suitably generalize it to cases where the Hamiltonian commutes with a global projection operator $P_{\mr{frag}}$  that fragments the Hilbert space. In the present case, we are interested in particular in the Rydberg constraint, i.e.,  $P_{\mr{frag}}=P_{\mr{Ryd}}$.
%i.e., $[H, P_{\mr{frag}}]=0$, 
Indeed, if $H$ possesses a generalized decomposition into a simple spectrum-generating part and an annihilator part, $H=H_{\mr{spec}}+H'_{\mr{ann}}$ (which do not need to commute with the fragmentation individually), the scar states %which we denote by $\ket*{\mc{S}_n}$ 
can be written as projections 
\begin{equation}
    \ket*{\mc{S}_n}=P_{\mr{frag}}\ket*{\wtil{\mc{S}}_n},
\end{equation} 
{\it provided} that  the parent state $\ket*{\wtil{\mc{S}}_n}$ is (i) an eigenstate of $H_{\mr{spec}}$ with energy $E_n$,
\begin{equation}
H_{\mr{spec}}\ket*{\wtil{\mc{S}}_n}=E_n\ket*{\wtil{\mc{S}}_n},
\end{equation} 
and (ii) is annihilated by $P_{\mr{frag}}H'_{\mr{ann}}$, 
\begin{equation}
P_{\mr{frag}}H'_{\mr{ann}}\ket*{\wtil{\mc{S}}_n}=0.    
\end{equation}
If these conditions are met, $\ket*{\mc{S}_n}$ is indeed an eigenstate of $H$ with energy $E_n$. The framework we outlined in the introduction %i.e., $H=H_{\mr{spec}}+H_{\mr{ann}}$ 
can then be understood as the special case where $P_{\mr{frag}}$ is simply the identity operator. 

As we found empirically above, the "Lie algebra-modified" PXP model, $H_{\mr{mod}}=H+\delta H_{\mr{Lie}}$, approximately possesses such a generalized decomposition, with the  spectrum generating Zeeman term $H_{\mr{spec}}=H_{\mr{Z}}$ and a generalized (approximate) annihilator $H'_{\mr{ann}}\equiv H_{\mr{mod}}-H_{\mr{Z}}=H_1+H_2+\delta H_{\mr{Lie}}$. This observation clarifies in what sense the PXP chain can be understood as being close to a model that shares the common general structure of most other known scar-hosting models.

%\MM{I don't fully understand the following paragraph}
%\blue{The revealed structure \MM{which one?} rationalizes the fact that our ansatz $\ket*{S_n}$ has a high overlap with the exact scar states. Indeed, we can find for several different lattices,}
%\begin{equation}\label{eq:mechanism}\begin{split}
    %\blue{H\ket*{S_n}}&\blue{=P_{\mr{Ryd}}\left(H_{\mr{Z}}+H_1+H_2\right)\ket*{\wtil{S}_n}}\\
    %&\blue{=n\sqrt{2}\ket*{S_n}+P_{\mr{Ryd}}H_1\ket*{\wtil{S}_n}}\\
    %&\blue{\approx\left(n\sqrt{2}+\Delta E_n\right)\ket*{S_n},}
    %\end{split}
%\end{equation}
%\blue{where $\Delta E_n \MM{= ...}$ is an energy correction due to $H_1$, while the contribution from $H_2$ vanishes, since $P_{\mr{Ryd}}H_2=0$. From this we conjecture that the PXP model on a bipartite lattice has scar states when the  component of $P_{\mr{Ryd}}H_1\ket*{\wtil{S}_n}$ orthogonal to $\ket*{S_n}$ is small. \MM{Moreover the tower of states is nearly equidistant, if the $\Delta E_n$ only weakly depend on $n$.} This suggests that lattices with the small coordination number might be good candidates, as the number of terms in $H_1$ increases with the coordination number.}

%\blue{Furthermore, Eq.~\eqref{eq:mechanism} yields}
\section{Exact scars in a non-Hermitian PXP extension and connections with Hermitian perturbations}
\label{sec:exact perturbation}
The observation that projections of maximal spin states are close to the actual scar states suggests how one could construct a  modification of the PXP model having the states $\ket{S_n}$ as {\it exact} scar eigenstates. One simply needs to find a (potentially non-Hermitian) perturbation $H\to H +\delta H_{\mr{NH}}$ which satisfies $P_{\mr{Ryd}}(H_1+\delta H_{\mr{NH}})\ket*{\wtil{S}_n}=0$ for $\forall n$, taking into account that $P_{\mr{Ryd}}H_2=0$. 
We recall that $\ket*{\wtil{S}_n}$ is a maximal spin state, and thus is annihilated by the operators ${1-P_{b,b_1,\cdots,b_k}^{S=k+1}}$, which project out the maximal spin sector  {($S=k+1$) of any set of $k+1$} block spins. Below we will focus on sets consisting of $b$ and the $k$ blocks $b_1,...,b_k$ that are connected by an edge to one of the vertices of $b$). We thus may seek $\delta H_{\mr{NH}}$ such that {$(H_1+\delta H_{\mr{NH}})\prod_bP^{S=k+1}_{b,b_1,\cdots,b_k}=0$}.  
We thus construct an operator that neutralizes the action of $H_1$ on the maximal spin states. 
Eq.~\eqref{eq:pxp block-basis} shows that $H_1$ is a sum of operators, each acting on a block $b$ and the $k$ neighbors of one of its vertices. %\MM{write it out explicitly, and give the states that appear there a name}
We now construct a neutralizing counterterm for each one of these.  This can be achieved by the choice %\MM{I WOULD change the notation ${\{d_i\}_i}\to {\{d_i\}}$, or is there a reason for it?}
\begin{equation}\label{eq:noneq-pert condition}\begin{split}
{\delta H_{\mr{NH}}}&{=-\sum_{b\in\Lambda_{\mr{B}}}\left(\sum_{k=1}^{z_{b_\alpha}-1}(-1)^k\delta h^{k;\alpha}_b+\sum_{k=1}^{z_{b_\beta}-1}(-1)^k\delta h_b^{k;\beta}\right)}\\
{\delta h_b^{k;\alpha}}&{=\sum_{\substack{\{c_i\}_{i=1}^k\subset\Lambda_{\mr{B}}\\(c_i)_\beta\in\partial b_\alpha\setminus\{b_\beta\}}}\dyad*{0,-,\cdots,-}{\chi_{\{c_i\}}^\alpha}_{b,c_1,\cdots,c_k}}\\
{\delta h_b^{k;\beta}}&{=\sum_{\substack{\{d_i\}_{i=1}^k\subset\Lambda_{\mr{B}}\\(d_i)_\alpha\in\partial b_\beta\setminus\{b_\alpha\}}}\dyad*{0,+,\cdots,+}{\chi_{\{d_i\}}^\beta}_{b,d_1,\cdots,d_k},}%\blue{=-\sum_{b\in\Lambda_{\mr{B}}}\sum_{k=1}^{z_{b_\alpha}-1}(-1)^k\dyad*{0,+,\cdots,+}{\chi_+}_{b,b_1,\cdots,b_k}},
\end{split}
\end{equation}
where {$\ket*{\chi_{\{c_j\}}^\alpha}$ and $\ket*{\chi^\beta_{\{d_j\}}}$} are any wavefunctions of the {($k+1$)} blocks, that {satisfy} 
\begin{equation}\label{eq:counter}
    \begin{split}
        {P_{b,c_1,\cdots,c_k}^{S=k+1}\left(\ket*{\chi_{\{c_i\}}^\alpha}-\ket*{+,-,\cdots,-}\right)_{b,c_1,\cdots,c_k}}&{=0},\\
        {P_{b,d_1,\cdots,d_k}^{S=k+1}\left(\ket*{\chi^\beta_{\{d_i\}}}-\ket*{-,+,\cdots,+}\right)_{b,d_1,\cdots,d_k}}&{=0.}
    \end{split}
\end{equation}
{Indeed, the terms $\delta h_b^{k;\alpha}$ ($\delta h_b^{k;\beta}$) compensate the action of $h_b^{k;\alpha}$ ($h_b^{k;\beta}$) in Eq.~\eqref{eq:H1 expanded} when acting on a maxinmal spin state, as is ensured by Eq.~\eqref{eq:counter}.}
%such that $\blue{P^{S=k+1}(\ket*{\chi_+}-\ket*{+,-})=0}$.

In addition, $\delta H_{\mr{NH}}$ should also  commute with $P_{\rm Ryd}$. This constrains the {$\ket*{\chi^{\alpha,\beta}}$} further, requiring {$\dyad*{-}_b\ket*{\chi^\alpha_{\{c_i\}}}=\dyad*{+}_b\ket*{\chi^\beta_{\{d_i\}}}=0$ and $\dyad*{+}_{c_j}\ket*{\chi^\alpha_{\{c_i\}}}=\dyad{-}_{d_j}\ket*{\chi^\beta_{\{d_i\}}}=0$ for $j=1,\cdots,k$.} These conditions  {potentially admit several solutions. Here we consider a simple one,} 
%\MM{You take a wavefunction having the same $S^z= k-1$, and then you make sure that the scalar products with the state $\ket*{S=k+1,S^z=k-1}$ of the two wavefunctions in (24) is the same }
\begin{equation}
    \begin{split}
        {\ket*{\chi^\alpha_{\{c_i\}}}_{b,c_1,\cdots,c_k}}&={\frac{1}{2k}\sum_{j=1}^k\ket*{0,-,\cdots,\underbracket[1pt][1pt]{0}_{c_j},\cdots,-}_{b,c_1,\cdots,c_k}}\\
        {\ket*{\chi^\beta_{\{d_i\}}}_{b,d_1,\cdots,d_k}}&{=\frac{1}{2k}\sum_{j=1}^k\ket*{0,+,\cdots,\underbracket[1pt][1pt]{0}_{b_j},\cdots,+}_{b,d_1,\cdots,d_k},}
    \end{split}
\end{equation}
where the bracket indicates that the configuration of block $c_j(d_j)$ in $\ket*{\chi^\alpha}(\ket*{\chi^\beta})$  is $\ket*{0}$, while all other blocks $c_m(d_m)\,\,(m\neq j)$ are in state $\ket*{\pm}$.
The state $\ket*{\chi^\alpha}(\ket*{\chi^\beta})$ is chosen to have the same total spin projection $S^z=k-1$ $(S^z=-k+1)$, as the states $\ket*{+,-,\cdots,-}$ $(\ket*{-,+,\cdots,+})$ appearing in Eq.~\eqref{eq:counter}.
Moreover, we choose them such that their inner product with the state $\ket*{S=k+1,S^z=k-1}(\ket*{S=k+1,S^z=-k+1})$ be the same as that of the states $\ket*{+,-,\cdots,-}(\ket*{-,+,\cdots,+})$. This then establishes that Eq.~\eqref{eq:counter} holds.
%the unique solution $\ket*{\chi}= \frac{1}{2}\ket{0,0}$.

The above construction ensures that the extended non-Hermitian model $H_{\mr{NH}}= H+\delta H_{\mr{NH}} \equiv H_Z+ H_{\rm ann}'$ possesses exact, energy-equidistant scar states $\ket*{S_n}=P_{\mr{Ryd}}\ket*{\wtil{S}_n}$ since (i) $H_{\mr{NH}}$ commutes with $P_{\mr{Ryd}}$, %(ii) $H_2$ is annihilated by $P_{\mr{Ryd}}$, i.e., $P_{\mr{Ryd}}H_2=0$, and (iii) 
(ii) the parent states $\ket*{\wtil{S}_n}$ are eigenstates of $H_Z$ and (iii) they are annihilated by $P_{\mr{Ryd}} H_{\rm ann}'= P_{\mr{Ryd}}(H_1+\delta H_{\mr{NH}})$, as ensured by Eq.~\eqref{eq:counter}. 
{The resulting non-Hermitian modification of the PXP model having an exact, energy-equidistant tower of scar states, can be cast into the generalized projector-embedding form}{: For any state $\ket*{\psi}\in\mb{C}^{3\otimes N_b}$, the perturbed Hamiltonian acts on its Rydberg projected component $P_{\mr{Ryd}}{\ket*{\psi}}$} as 
\begin{equation}\label{eq:generalized pe}\begin{split}
    &{\left(H+\delta H_{\mr{NH}}\right)P_{\mr{Ryd}}}{\ket*{\psi}}\\&{=P_{\mr{Ryd}}\left[H_{\mr{Z}}+\sum_{b\in\Lambda_{\mr{B}}}h_b\left(1-P_b^{S=S_{\mr{max}}}\right)\right]}{\ket{\psi},}
    \end{split}
\end{equation}
{where $1-P_b^{S=S_{\mr{max}}}$ is a local projector annihilating the parent states of the scars.}

{We recall that the scar states $\ket*{S_n}$ are invariant under a change of the dimerization used to construct the parent states. This can be used to symmetrize $\delta H_{\mr{NH}}$ and restore the symmetries that were lost by the choice of dimerization (see Appendix.~\ref{sec:appendix inv perturbation} for a detailed discussion). Below we carry this out  explicitly for the chain.} 

\subsubsection{{One-dimensional chain}}\label{sec:1D perturbation}
{For the 1D chain, there is only $k=1$ block neighboring a given vertex, and the above construction yields {$\ket*{\chi^{\alpha,\beta}}=\ket*{0,0}$}. {From Eq.~\eqref{eq:noneq-pert condition}} we see that $\delta H_{\mr{NH}}$ then takes the form} 
\begin{equation}\begin{split}
    {\delta H_{\mr{NH}}}&{=\frac{1}{2}\sum_{b\in\Lambda_{\mr{B}}}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{0,0}_{b,b+1}}\\
    &{=\frac{1}{2}\sum_{b\in\Lambda_{\mr{B}}}P_{2b-1}\left(\sigma^+_{2b}P_{2b+1}+P_{2b}\sigma^+_{2b+1}\right)P_{2b+2},}
    \end{split}
\end{equation}
{where $\sigma^+\coloneqq\dyad*{\uparrow}{\downarrow}$. Here we express $\delta H_{\mr{NH}}$ in the basis of the original $S=1/2$ degrees of freedom {whereby the bond $b$ is formed by the sites $(2b-1, 2b)$}. From this we can obtain an associated  translationally invariant perturbation $\delta H^{\mr{inv}}_{\mr{NH}}$ by averaging $\delta H_{\mr{inv}}$ over translations}
\begin{equation}\begin{split}
\label{Hinv}
    {\delta H^{\mr{inv}}_{\mr{NH}}}&{=\frac{1}{2}\left(\delta H_{\mr{NH}}+ T^{-1}\delta H_{\mr{NH}}T\right)}\\
    &{=\frac{1}{4}\sum_{i\in\Lambda}P_{i-1}\sigma^+_iP_{i+1}\left(P_{i-2}+P_{i+2}\right).}
    \end{split}
\end{equation}
{which still satisfies the requirements (i)-(iii). Moreover,}
{$\ket*{S_n}$ is still an exact eigenstate of $H+\delta H^{\mr{inv}}_{\mr{NH}}$, since $\ket*{S_n}$ is translational invariant.} %ear by construction that $H$ and $H+\delta H^{\mr{inv}}_{\mr{NH}}$ are continuously connected in the sense that a family of the operator $H(\tau)=H+\tau\delta H^{\mr{inv}}_{\mr{NH}}$ with $\tau\in[0,1]$ has a set of eigenstates that are well-approximated by $\ket*{S_n}$. This fact should be contrasted to Ref.~\cite{PhysRevB.105.245137} in which the authors found the exact $SU(2)$ algebra only in a model that is not smoothly connected to the PXP model.}

\subsubsection{{Honeycomb lattice}}\label{sec:honeycomb perturbation}
{For the honeycomb lattice, $\delta H_{\mr{NH}}$ becomes}
\begin{equation}
    \begin{split}
        {\delta H_{\mr{NH}}}&{=\frac{1}{2}\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\sum_{i=1,2}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{0,0}_{\Vec{R},\Vec{R}+\Vec{e}_i}}\\
        &{-\frac{1}{4}\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\ket*{0,-,-}\left(\bra*{0,0,-}+\bra*{0,-,0}\right)_{\Vec{R},\Vec{R}+\Vec{e}_1,\Vec{R}+\Vec{e}_2}}\\
        &{-\frac{1}{4}\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\ket*{+,+,0}\left(\bra*{0,+,0}+\bra*{+,0,0}\right)_{\Vec{R}-\Vec{e}_1,\Vec{R}-\Vec{e}_2,\Vec{R}}.}
    \end{split}
\end{equation}
{Again, we can obtain a rotationally invariant perturbation $\delta H_{\mr{NH}}^{\mr{inv}}$ by averaging $\delta H_{\mr{NH}}$ over rotations (see Appendix.~\ref{sec:appendix inv perturbation}).}



It would obviously be very challenging to engineer an open system with effective non-Hermitian terms Eq.~(\ref{eq:noneq-pert condition}).  However, the main purpose of our  construction is to explicitly show  that the PXP model is in fact close to a model with a strictly local Hamiltonian that preserves the Rydberg constraint and possesses a tower of exact scar states. 
Moreover our explicit example furnishes an illustration of the general algebraic structure underlying scars in a system with a constraint $P_{\mr{Ryd}}$ that fragments Hilbert space.

\subsection{Hermitian scar enhancements of $H_{\rm PXP}$}

A drawback of the above discussed modification is that $H_{\mr{NH}}$ is non-Hermitian. We may, however, take it as a starting point to seek a {\it Hermitian} scar-enhancing perturbation $\delta H$. This will establish a connection to perturbations that have been proposed previously in the literature for the 1D chain.  

%A natural ansatz for a Hermitian perturbation 
%$\delta H(\lambda)$ by adding $H^\dag_{\mr{NH}}$:
%\begin{eqnarray}\label{eq:dH(lambda)}
%\begin{split}
%    &&\delta H(\lambda)\coloneqq\green{\lambda}\left(\delta H_{\mr{NH}}+\delta H_{\mr{NH}}^\dag\right)\\
%   &&\quad=\green{\frac{\lambda}{2}}\sum_{b\in\Lambda_{\mr{B}}}\Big(\left(\ket{+,0}+\ket{0,-}\right)\bra{0,0}+\ket{0,0}\left(\bra{+,0}+\bra{0,-}\right)\Big)_{b,b+1}\nonumber
 %    \end{split}
%    \end{eqnarray}
%    where we allow the coefficient $2\lambda$ \MM{??} to differ from $1$ \MM{but if $\delta H_{\mr{NH}}$ were Hermitian, we would say that $2\lambda$ should be 1/2, not 1. Do you find it more reasoanble to compare with 1? 1/2 would be much closer to what we find later. I  don't quite understand why we don't write $\lambda/2$ as prefactor, so we can translate everything later to umbers that should be compared to 1}, so as to correct for the fact that $P_{\mr{Ryd}}\delta H_{\mr{NH}}^\dag$ does not annihilate  $\ket*{\wtil{S}_n}$ and thus introduces uncompensated terms in the eigenvalue equation for the supposed scar state $\ket{S_n}$.  
%An interesting relation with previous approaches appears when we express $\delta H(\lambda)$ in the basis of the original $S=1/2$ degrees of freedom, 
%\begin{equation}\label{eq:dH2(lambda)}    
%    \delta H(\lambda) =\green{\frac{\lambda}{2}}\sum_{b\in\Lambda_{\mr{B}}}\left(P_{2b-1}X_{2b}P_{2b+1}P_{2b+2}+P_{2b-1}P_{2b}X_{2b+1}P_{2b+2}\right).
%\end{equation}

%\MM{MY SUGGESTION:} 
Since the non-Hermitian Hamiltonian has real eigenvalues on the scar states, the have vanishing expectation values for its imaginary part.
Thus, an obvious ansatz for a Hermitian perturbation is simply the real part of $\delta H^{\mr{inv}}_{\mr{NH}}$ in Eq.~(\ref{Hinv}),
\begin{equation}\label{eq:dH2new(lambda)}    
    \delta H(\lambda) =\frac{\lambda}{2}(\delta H^{\mr{inv}}_{\mr{NH}}+\delta H^{\mr{inv}\dagger}_{\mr{NH}})
    ={\frac{\lambda}{8}}\sum_{i\in\Lambda}P_{i-1}X_{i}P_{i+1}(P_{i-2}+P_{i+2}).
\end{equation}
where we allow for a coefficient $\lambda\neq 1$ to optimize the resulting Hamiltonian. This is precisely the perturbation studied in Refs.~\cite{nearly_su2, Kieran2020}. 
%In view of the translation invariance of $H$ and the targeted scar states $\ket*{{S}_n}$ it is natural to average $\delta H(\lambda)$ over translations. %and erasing the trace of our arbitrary choice of forming block spins,
%This systematic construction results in the perturbation $\delta H_{\rm inv}=(\lambda/\green{4})\sum_{i\in\Lambda}P_{i-1}X_iP_{i+1}(P_{i-2}+P_{i+2})$, 
%where $\lambda$ is a coefficient, and we also express it in the spin-$1/2$ basis in the last line. Due to the presence of $H_{\mr{NH}}^\dag$, $\delta H(\lambda)$ does not make $\ket{S_n}$ exact eigenstate at $\lambda=1/2$, i.e., $P_{\mr{Ryd}}(H_1+\delta H(1/2))\ket*{\wtil{S}_n}=P_{\mr{Ryd}}H_{\mr{NH}}^\dag\ket*{\wtil{S}_n}$. Thus it is natural to introduce the parameter $\lambda$ so that $\delta H(\lambda)$ partially cancels $H_1$ by $2\lambda H_{\mr{NH}}$ ($P_{\mr{Ryd}}(H_1+2\lambda H_{\mr{NH}})\ket*{\wtil{S}_n}$), while $2\lambda P_{\mr{Ryd}}H_{\mr{NH}}^\dag\ket*{\wtil{S}_n}$ should be kept small. Note that $\delta H(\lambda)$ is close to the perturbations appearing in Refs.~\cite{nearly_su2, Kieran2020}. Indeed, by adding a shifted operator of $\delta H(\lambda)$, one can get $\lambda\sum_{i\in\Lambda}P_{i-1}X_iP_{i+1}(P_{i-2}+P_{i+2})$. 
It remains to optimize $\lambda$ such that the $\ket*{{S}_n}$ become as close as possible to exact eigenstates. To this end we minimize
$\sum_{n=1}^N\norm*{P_{\mr{Ryd}}(H_{1}+\delta H(\lambda))\ket*{\wtil{S}_n}}^2$.
If we neglect the projection by $P_{\mr{Ryd}}$ the minimization can be carried out analytically in the large $N_b$ limit, yielding $\lambda\approx 1.02$. %0.2651
%0.1325$.
Numerical minimization including the projector instead yields the slightly smaller value $\lambda^*\approx%0.2329 %0.1165
0.93$ (for $N_b=10$), 
which is close to the values obtained with different optimization criteria in Refs~\cite{nearly_su2,Kieran2020}.
With the thus optimized Hamiltonian $H+\delta H(\lambda^*)$ the overlap between the exact and our approximate scar wavefunctions is very high: for $N_b=10$ we find $|\innerproduct*{\mc{S}^{\mr{PXP}}_n}{S_n}|^2\gtrsim 0.95$, cf. Fig.~\ref{fig:<Sn|Sn> squared}. 

The above again confirms the hidden structure of the scar states in both the PXP model and its scar-enhanced cousins: They are projected maximal spin states, as pictorially illustrated in Fig.~\ref{fig:illustration}. Thereby, the large spin $S_{\rm tot}=N_b$ is composed of $N_b$  block spins $S=1$ formed by two elementary $S=1/2$. The N\'eel state has $S^z_{\rm tot}=N_b$ and thus corresponds to the large spin lying essentially in the equatorial plane with respect to the Zeeman field $\sqrt{2}$ along $e_x$, having approximately $S^x_{\rm tot}\approx 0$. 
%\MM{move up}
%Interestingly, after Rydberg projection, either choice of dimerization to form block spins results in identical scar states. These thus provide equivalent descriptions of the PXP dynamics, even though the parent states $\ket*{\what{S}_n}$ slightly differ and are not translationally invariant in the original basis of $S=1/2$ spins. 
%This is a consequence of the fact that $\ket*{S_n}$ is numerically found to be invariant under translation by \textit{one spin-$1/2$ site}. %(Unlike in Motrunich's MPS) 
Upon initialization in the Néel state or elsewhere close to the scar subspace, the dynamics of the system is explicitly seen to be the precession of the large pseudo-spin around its $x$-axis, whose motion is projected down from the $3N$-dimensional $S=1$ space onto the smaller constrained space ${\cal V}_{\rm Ryd}$, cf.~Fig.~\ref{fig:illustration}. Up to small corrections the precession frequency is set by the coefficient $\sqrt{2}$ of the Zeeman term in the $S=1$ space. 

 %We find that $P_{\mr{Ryd}}\left(H_1+\delta H(\lambda)\right)\ket*{\wtil{S}_n}=P_{\mr{Ryd}}H_{\mr{rem}}(\lambda)\ket*{\wtil{S}_n}$, where
%\begin{equation}
 %   \begin{split}
  %      H_{\mr{rem}}(\lambda)&=\sum_{b\in\Lambda_{\mr{B}}}h_{b,b+1}(\lambda)\\
   %     h_{b,b+1}(\lambda)&\coloneqq\frac{-1+2\lambda}{\sqrt{6}}\left(\ket{+,0}+\ket{0,-}\right)\bra*{T_{2,0}}_{b,b+1}\\
    %    &+\frac{\lambda}{\sqrt{2}}\ket{0,0}\left(\bra*{T_{2,1}}+\bra*{T_{2,-1}}\right)_{b,b+1}.
%    \end{split}
%\end{equation}
%To obtain this we subtract irrelevant terms of a form $\dyad*{\psi}{T_{S,M}}\,\,(S<2)$ from $H_1+\delta H(\lambda)$, as they must annihilate $\ket*{\wtil{S}_n}$. The second line in the right-hand side and the third line correspond to $H_1+2\lambda H_{\mr{NH}}$ and $2\lambda H^\dag_{\mr{NH}}$ followed by subtracting irrelevant terms. 
%One can roughly estimate the optimal coefficient $\lambda$ by requiring that $h_{b,b+1}(\lambda)\ket*{\wtil{S}_n}$ be small. We find that when $N$ is large enough, this function is minimized at $\lambda\approx 0.2651$. See Supplemental Material for a derivation of this value. 

%\textit{A sequence of Hermitian perturbations.}--From the non-Hermitian perturbation, we can construct a sequence of Hermitian perturbations which make $\ket{S_n}$ asymptotically exact. If we do not impose the condition in Eq.~\eqref{eq:noneq-pert condition} that $\left(\ket{+,0}+\ket{0,-}\right)\bra{\chi}$ should commute with $P_{\mr{Ryd}}$, but a more relaxed one that $\ket{\chi}$ should not include $\ket{+,-}$, the choice of $\ket{\chi}$ is not unique. Namely, $\ket{\chi}=\frac{1-a}{2}\ket{0,0}+a\ket{-,+}$ with a coefficient $a$ satisfies it. The norm $\norm{\ket{\chi}}\coloneqq\sqrt{\innerproduct{\chi}}$ is minimized when $a=1/5$. Then, we define 
%\begin{equation}
    %H'_1=\frac{1}{5}\sum_{b\in\Lambda_{\mr{B}}}\left(\ket{+,0}+\ket{0,-}\right)\left(2\bra{0,0,}+\bra{-,+}\right)_{b,b+1}.
%\end{equation}
%We make $H'_1$ commute with $P_{\mr{Ryd}}$ by adding $(1-\dyad{-})_{b+2}$ and $(1-\dyad{-})_{b-1}$. Namely we define 
%\begin{equation}
    %\begin{split}
        %H_1&=\frac{2}{5}\sum_{b\in\Lambda_{\mr{B}}}\left(\ket{+,0}+\ket{0,-}\right)\bra{0,0}_{b,b+1}\\
        %+&\frac{1}{5}\sum_{b\in\Lambda_{\mr{B}}}\left(1-\dyad{+}\right)_{b-1}\left(\ket{+,0}+\ket{0,-}\right)\bra{-,+}_{b,b+1}\\
        %&\qquad\otimes\left(1-\dyad{-}\right)_{b+2}.
    %\end{split}
%\end{equation}
%Our ``first-order" Hermitian perturbation is thus $\delta_1H\coloneqq H_1+H^\dag_1$. $H_{\mr{anil}1}$ is canceled by a part of $H_1$, but the rest of $H_1$ and $H^\dag_1$ could contain terms not annihilating $\ket*{\wtil{S}_n}$, which we denote by $\delta_1H_{\mr{anil}1}$. However, the coefficient of $\delta_1H_{\mr{anil}1}$ becomes smaller. We can repeat the same procedure for $\delta_1H_{\mr{anil}1}$, which might produce another non-annihilating terms $\delta_2H_{\mr{anil}1}$ with even smaller coefficients. Thus, our recipe to get a sequence of Hermitian perturbations is summarized as follows:
%\begin{itemize}
    %\item[step $1$] for a given $H_k\,\,\,(k\in\mb{N})$, calculate $H_k^\dag$. Here we assume $H_k^\dag=\sum_{b\in\Lambda_{\mr{B}}}\sum_\mu \lambda_\mu\dyad{\varphi_\mu}{\psi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$ where $\dyad{\varphi_\mu}{\psi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$ is a $i_{k,\mu}$-body operator acting on sites $b,\cdots,b+i_{k,\mu}-1$. Here $\mu$ labels different terms and $\lambda_\mu$. is a coefficient. We assume that $\ket*{\psi_\mu}$ is a product state. 
    %\item[step $2$] expand $\ket{\psi_\mu}$ with respect to a composite spin basis $\ket*{T_{S,M}}$, i.e., $\ket{\psi_\mu}=\sum_S^{i_{k,\mu}}\sum_{M=-S}^Sc_{S,M}\ket*{T_{S,M}}$. We should find a state $\ket{\chi_\mu}=\sum_S^{i_{k,\mu}}\sum_{M=-S}^Sd_{S,M}\ket*{T_{S,M}}$ such that $d_{i_{k,\mu},M}=c_{i_{k,\mu},M}$ for $\forall M$ and $\ket*{\chi_\mu}$ does not contain $\ket{+,-}$ anywhere. If there is multiple choices for $\ket{\chi_\mu}$, we choose $\ket{\chi_\mu}$ with the minimum norm. %$\dyad{\varphi_\mu}{\chi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$ commutes with $P_{\mr{Ryd}}$.
    %\item[step $2a$] if (except for $\ket{\psi_\mu}$ itself) there is no $\ket{\chi_\mu}$ satisfying the condition on $d_{S,M}$ above, we should insert the identity operator $id_{b+i_{k,\mu}}=\dyad{+}+\dyad{0}+\dyad{-}$, i.e., $\sum_{\alpha=\pm,0}\dyad{\varphi_\mu}{\psi_\mu}_{b,\cdots,b+i_k-1}\dyad{\alpha}{\alpha}_{b+i_{k,\mu}}$, and for each $\ket{\psi_\mu}\ket{\alpha}$ we repeat step $2$.
    %\item[step $2b$] if $\dyad{\varphi_\mu}{\chi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$ constructed in step $2$ (and $2a$) does not commute with $P_{\mr{Ryd}}$, we should add operator $\left(1-\dyad{-}\right)_{b+i_{k,\mu}}$ and/or $\left(1-\dyad{+}\right)_{b-1}$, i.e.,  $\dyad{\varphi_\mu}{\chi_\mu}_{b,\cdots,b+i_{k,\mu}-1}(1-\dyad{-})_{b+i_{k,\mu}}$ or $(1-\dyad{+})_{b-1}\dyad{\varphi_\mu}{\chi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$.
    %\item[step $3$] define $H_{k+1}\coloneqq-\sum_{b\in\Lambda_{\mr{B}}}\sum_\mu\lambda_\mu\dyad{\psi_\mu}{\chi_\mu}_{b,\cdots,b+i_{k,\mu}-1}$ and we obtain a perturbation $\delta_{k+1}H\coloneqq H_{k+1}+H_{k+1}^\dag$.
%\end{itemize}
%We show that perturbations obtained in this procedure should have a vanishing coefficient as $k\rightarrow\infty$ in supplemental material. Note that this procedure would yield exponentially many perturbations. 

==> phenomenology.tex <==
\label{sec:phenomenology}
%We first summarize a generic structure that is common to almost all models with scar states.
%The term ``many-body scar" was introduced in the context of the quasi-periodic dynamics of the PXP model~\cite{Turner2018}, to emphasize the analogy to quantum scars in single particle billiards~\cite{quantum_scar_original}. However, the feature that sticks out in  models~\cite{tos_aklt,tos_xy,tos_exact_2,Lin2020,Kiryl2020,Kiryl2021} exhibiting exactly periodic quantum dynamics is not the concentration of Wigner functions on classical periodic orbits, but rather the existence of a tower of energetically exactly equidistant eigenstates with low entanglement entropy, the so-called scar states.
The existence of scar states, nonthermal eigenstates in systems with a non-integrable Hamiltonian, is a consequence of a structure common to almost all models with analytically known towers of exact scar states~\cite{tos_aklt_unified, KO2022}%\MM{citation to Motrunich and our 2nd paper needed here!}
: The Hamiltonian $H$ can be split into two parts, $H=H_{\mr{spec}}+H_{\mr{ann}}$. The scar states, denoted by $\ket{\mc{S}_n}$, are eigenstates of $H_{\mr{spec}}$ with equidistant eigenenergies %~\footnote{Note that one can obtain non-ergodic states even when $H_{\mr{spec}}=0$, but we do not call them scar states, as an initial states consisting of such states does not exhibit revivals, which is an essential feature of QMBS.}
%($H_{\mr{spec}}\ket{\mc{S}_n}=E_n\ket{\mc{S}_n}$) 
$E_n$ [i.e., $(E_n-E_m)/\Omega \in \mathbf Z$],  
and are annihilated by $H_{\mr{ann}}$ ($H_{\mr{ann}}\ket{\mc{S}_n}=0$). Both $H_{\mr{spec}}$ and $H_{\mr{ann}}$ are local in the sense that they are sums of local operators. Any superposition of $\ket{\mc{S}_n}$ exhibits exact revivals under unitary time evolution by multiples of $1/\Omega$ ($\hbar =1$). $H_{\mr{spec}}$ {is integrable and }often consists in a simple Zeeman term% or a sum of mutually commuting terms such as Ising interactions
~\cite{tos_xy, tos_exact_2}. %\MM{\it which is a Zeeman term upon a site-to bond transformation}~\cite{tos_xy, tos_exact_2}.
$H_{\mr{ann}}$ renders the remainder of the spectrum chaotic. In most cases it can be further decomposed into scar-annihilating {\em local} operators. Sets of such local annihilators that have a non-trivial common kernel (namely the prospective scar states) can be systematically constructed~\cite{mori_shiraishi, Kiryl2020, Kiryl2021, Ren2021Quasisymmetry}. An instructive example is the projector-embedding by Shiraishi and Mori~\cite{mori_shiraishi}.   %the Shiraishi-Mori construction~\cite{mori_shiraishi}. 
{In this approach, $H_{\mr{ann}}$ is written as $H_{\mr{ann}}=\sum_i\mc{P}_ih_i\mc{P}_i$, where $\mc{P}_i$ is a local projector and $h_i$ is any local operator. Scar states are annihilated separately by every $\mc{P}_i$. For various models, such a decomposition of the Hamiltonian has been identified, although sometimes one has to enlarge the Hilbert space to find local annihilators~\cite{KO2022}.} %An interesting example is the Affleck-Kennedy-Lieb-Tasaki (AKLT) model, where $H_{\mr{spec}}$ is a Zeeman term. However, the remainder $H_{\mr{ann}}$ can be decomposed into local annihilators only when the Hilbert space is enlarged~\cite{KO2022}. 
{However, previous attempts~\cite{nearly_su2,Iadecola2019pimagnon,Lin2019mps,Khemani2019integral} to understand the scar states in the PXP model have not succeeded to uncover a similar structure in the Hamiltonian, which has hindered a unified understanding of the nature of the QMBS appearing in PXP models and of the way in which they relate to the analytically known QMBS in other systems.} Here, we will close this gap by showing how the {PXP model} fits within such a framework {: It can be approximately expressed in a \textit{generalized} projector-embedding form,}
\begin{equation}
    {HP_{\mr{Ryd}}{\ket*{\psi}}\approx P_{\mr{Ryd}}\left(H_{\mr{Z}}+\sum_ih_i\mc{P}_i\right){\ket*{\psi}},}
\end{equation}
{where $P_{\mr{Ryd}}$ imposes the Rydberg blockade condition that prohibits simultaneous excitations of neighboring atoms, a precise definition being given further below in Eq.~\eqref{eq:projector}. $H_{\mr{Z}}$ turns out to be a simple Zeeman term, while $H_{\mr{ann}}=\sum_ih_i\mc{P}_i$ annihilates states of  maximal total spin, once $H$ is expressed in a basis of $S=1$ ``block-spins", each of which describes the Rydberg-allowed configurations of two neighboring $S=1/2$ spins.} Note that the operator on the right-hand side (RHS) acts on the partially restricted 
%\sout{full (non-restricted $S=1/2$)} 
Hilbert space of {block spins} and is non-Hermitian, while the Hamiltonian on the left-hand side (LHS) acts essentially in the space that satisfies the Rydberg constraint. Such a non-Hermiticity often arises when the action of a Hamiltonian is lifted to a Hilbert space of larger dimension. Indeed a similar structure, arises in the AKLT model when one tries to understand its scar states in terms of local annihilators ~\cite{KO2022}.

% Is this necessary?
%\MM{\it I would say this in the conclusion, not here} We also note that scar states can often be understood as a ``lift" of spin-$1/2$ states~\cite{KO2022}. One can define a suitable subspace which is isomorphic to the spin-$1/2$ Hilbert space, and the scar states, after a suitable unitary transformation, become highly symmetric states. Local annihilating terms in $H_{\mr{ann}}$ consist of projectors which project out the scar states. Interestingly, we will see that the scar states in the PXP model are \textit{not} mapped to such spin-$1/2$ states.    
%For $H_1$, one possible choice is a sum of generators of certain symmetry~\cite{Kiryl2020,Kiryl2021}, i.e., $H_1=\sum_iO_iT_i$ where $T_i$ is a generator of some group and $O_i$ makes $O_iT_i$ Hermitian. In this case, scar states are one dimensional representations of the corresponding symmetry. We emphasize that each generator can be a local operator and annihilates the scar states, i.e., $T_i\ket{S_n}=0$ for $\forall i$. 

%In the following sections, we show that well-known models hosting scar states have the above-mentioned structures. More precisely, we claim that the Hamiltonian $H$ is expressed as
%\begin{equation}\label{eq:basic scheme}
   % H=\sum_iS_i+\sum_iP_i=H_0+H_1.
%\end{equation}
%The first term $\sum_iS_i$ corresponds to $H_0$ above, which is responsible for the equidistant energies and thus we call it the spectrum-generating term. The second term consists of a local operator $P_i$ which annihilates scar states and thus we call it an annihilator. The locality of $S_i$ and $P_i$ is a crucial assumption. Eq.\eqref{eq:basic scheme} should be distinguished from the following trivial decomposition: for any set of eigenstates $\left\{\ket{\varepsilon_n}\right\}_n$, one can always write the Hamiltonian as
%\begin{equation}\label{eq:trivial decomposition}
    %H=\sum_n\varepsilon_n\dyad{\varepsilon_n}+\sum_{\ket{\epsilon_k}\not=\ket{\varepsilon_n}}\epsilon_k\dyad{\epsilon_k},
%\end{equation}
%where $\varepsilon_n$ is an energy of the target state $\ket{\varepsilon_n}$ and $\ket{\epsilon_k}$ is an eigenstate which does not belong to the target set with an energy $\epsilon_k$. This trivial decomposition might end up non-local operators. Thus Eq.\eqref{eq:trivial decomposition} is essentially different from Eq.\eqref{eq:basic scheme}.

%Also, scar states are often generated by a ``creation" operator $Q^\dag$ and a reference state $\ket{S_0}$ such that $\left(Q^\dag\right)^n\ket{S_0}=\mc{N}^{-1}\ket{S_n}$ with a normalization factor $\mc{N}$, particularly when they have equidistant energies. If there exists such an operator, we should require that $\left[H_0, Q^\dag\right]=\omega Q^\dag$ hold and $\left[H_1, Q^\dag\right]$ annihilate scar states~\cite{tos_aklt_unified}.


==> setup.tex <==
\label{sec:setup}
\subsection{Hamiltonian}
\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{lattice_general_PXP.eps}
    \caption{{Graphical representation of a bipartite lattice structure with its two sublattices $\Lambda_\alpha$ and $\Lambda_\beta$, colored in blue (dark grey) and red (light grey). The grey bars define a choice for a lattice of dimers, $\Lambda_{\mr{B}}$, each hosting a block spin.}}
    \label{fig:lattice}
\end{figure}
To describe a chain of Rydberg atoms with strong nearest neighbor repulsion between excited atoms Turner et al.~\cite{Turner2018} introduced the PXP model on a one-dimensional lattice. {Here we study this model and its generalization to a large class of bipartite lattices in arbitrary dimensions.}

{We consider an undirected graph $G=(\Lambda, E)$, where $\Lambda$ is a set of lattice sites (or vertices) and $E\subset\Lambda\times\Lambda$ is a set of edges labelled by their non-ordered endpoints, $(i,j) = (j,i) \in E$. Since $\Lambda$ is bipartite, there are two disjoint sublattices $\Lambda_\alpha$ and $\Lambda_\beta$ that cover the whole lattice ($\Lambda_\alpha\cup\Lambda_\beta=\Lambda$), and $(i,j)\in E$ implies either $i\in\Lambda_\alpha, j\in\Lambda_\beta$ or $i\in\Lambda_\beta, j\in\Lambda_\alpha$. Throughout most of this paper we assume $|\Lambda_\alpha|=|\Lambda_\beta|\equiv N_b$ (and thus $|\Lambda|=2N_b$). The PXP model on $\Lambda$ is defined as}
\begin{equation}\label{eq:pxp PBC}
	H=\sum_{i\in\Lambda}\left({X_i\prod_{j\,| (i,j)\in E}P_j}\right),
\end{equation} 
where $P\coloneqq\dyad{\downarrow}$ projects onto non-excited atoms while $X\coloneqq\dyad{\uparrow}{\downarrow}+\dyad{\downarrow}{\uparrow}$ drives the transition between ground and excited states. %Here, we assume periodic boundary condition (PBC), identifying site indices $i$ and $i+2N$. 
This Hamiltonian describes Rabi oscillations of individual atoms subject to the ``Rydberg" constraint  which requires  their neighboring atoms to be in their ground state, as implemented by the projectors $P$.

{We assume that $H$ is left invariant by the action of a crystalline symmetry group $G$, represented by operators $O_g$ that commute with $H$,  $[H, O_g]=0\,\forall g\in G$.}% For example, the 1D lattice with periodic boundary condition (PBC) has a symmetry group $G=\mb{Z}/\mb{Z}_{|\Lambda|}$.}%Here we do not consider the ``particle-hole" symmetry that anti-commutes with the Hamiltonian.}
{In the following, we focus on two examples: the one dimensional chain and the honeycomb lattice.}

\subsubsection{{One-dimensional chain}}
{For a one-dimensional chain, $\Lambda=\{1,\cdots,2{N_b}\}$ and $E=\{(i,i+1);\,i\in\Lambda\}$ with periodic boundary conditions ($i+2N_b\equiv i$). The Hamiltonian then becomes 
%what is commonly referred to as 'the' PXP model,
} 
\begin{equation}
    {H=\sum_{i\in\Lambda}P_{i-1}X_iP_{i+1}.}
\end{equation}
{In this case, the sublattices consist in the odd, $\Lambda_\alpha=\{2k+1;0\leq k\leq N_b-1\}$, and the even sites, $\Lambda_\beta=\{2k;1\leq k\leq N_b\}$, respectively. This model is  invariant under translation by one lattice spacing, which we denote by $T$, i.e., $[H,T]=0$. {The full lattice symmetry group also contains rotations around axes perpendicular to the chain, but those will not be of importance for our discussion.}} 

\subsubsection{{Honeycomb lattice}}
\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{honeycomb_lattice_exp.eps}
    \caption{Honeycomb lattice with its two sublattices $\Lambda_\alpha$ and $\Lambda_\beta$ coloerd in red (light grey) and blue (dark grey), respectively. The black arrows indicate $\Vec{e}_{1,2}$, the two basis vectors of the lattice used in the text.}
    \label{fig:honeycomb}
\end{figure}
{Another bipartite lattice of interest is the honeycomb lattice. To define the lattice $\Lambda$, it is easiest to directly define the sublattices $\Lambda_\alpha$ and $\Lambda_\beta$, namely, $\Lambda_\alpha=\{\Vec{r}=a_1\Vec{e}_1+a_2\Vec{e}_2;a_1,a_2\in\mb{Z}\}$ and $\Lambda_\beta=\{\Vec{r}+\Vec{e}_y;\Vec{r}\in\Lambda_\alpha\}$ where $\Vec{e}_{1,2}\coloneqq \pm\sqrt{3}/2\Vec{e}_x +\,3/2\Vec{e}_y$ are a set of basis vectors of $\Lambda_\alpha$ (see Fig.~\ref{fig:honeycomb}). We also implement PBC's, identifying $\Vec{r}$ and $\Vec{r}+N_i\Vec{e}_i$ for $i=1,2$ with some positive integers $N_i$. The PXP model on the honeycomb lattice is then defined as}
\begin{equation}\begin{split}
    {H}&{=\sum_{\Vec{r}\in\Lambda}X_{\Vec{r}}\prod_{\vec{r}'\in\partial\vec{r}}P_{\Vec{r}'},}
    \end{split}
%    &= \sum_{i\in \Lambda} X_i \prod_{j\in \partial i} P_j 
\end{equation}
{where $\partial\vec{r}\coloneqq\{\vec{r}'\in\Lambda|(\vec{r},\vec{r}')\in E\}$.}
{Note that the honeycomb lattice  is invariant under a site-centered rotation by an angle $2\pi/3$.}
\begin{comment}
\subsubsection{\blue{Decorated Bethe lattice}}
\blue{We also consider a rather artificial example which is based on the Bethe lattice. We construct the lattice $\Lambda$ by adding neighboring sites to the Bethe lattice. Namely, we consider the Bethe lattice with $M$ layers with the coordination number 3 except for the root (see Fig.~[FIG]). This lattice is three identical copies of a subset of the Bethe lattice. We define one of them as $\Lambda_\beta$. Thus, the condition $|\Lambda_\beta|=N$ implies the relation $2^M=N+1$. Each site in $\Lambda_\alpha$ is then placed in the middle of a line connecting neighboring nodes of $\Lambda_\beta$ (see Fig.~[FIG]). In this way, we can define a bipartite lattice $\Lambda(=\Lambda_\alpha+\Lambda_\beta)$ and the corresponding set of links $E$. The PXP model on this lattice is then,}
\begin{equation}
    \blue{H=\sum_{i\in\Lambda_\alpha}X_i\prod_{\substack{j\in\Lambda_\beta\\(i,j)\in E}}P_j+\sum_{i\in\Lambda_\beta}X_i\prod_{\substack{j\in\Lambda_\alpha\\(i,j)\in E}}P_j.}
\end{equation}
\blue{Note that we cannot impose the PBC in this case and the coordination number is not homogeneous.}
\end{comment}

\subsection{Dimerization}
The Hamiltonian {Eq.~\eqref{eq:pxp PBC}} commutes with the global projection operator $P_{\mr{Ryd}}\coloneqq\prod_{{(i,j)\in E}}(1-\dyad{\uparrow\uparrow})_{i,{j}}$ which prohibits neighboring atoms from being simultaneously excited. In the sequel we focus on the corresponding constrained subspace $\mc{V}_{\mr{Ryd}}\equiv P_{\mr{Ryd}}\mb{C}^{2\otimes2N_b}$. %{\mathcal H}$.
%\coloneqq\{\ket*{\Psi}|\ket*{\Psi}\in\mb{C}^{2\otimes N}, P_{\mr{Ryd}}\ket*{\Psi}=\ket*{\Psi}\}$. 
%\MM{drop?} whose dimension grows with $N$ as the Fibonacci sequence~\cite{Turner2018}. 
The constraint bars two neighboring spins from being up simultaneously. Hence, for the spins on an edge $b=(b_\alpha,b_\beta)$ {with neighboring sites $b_\alpha\in\Lambda_\alpha$ and $b_\beta\in\Lambda_\beta$},
only three configurations are possible.
%, namely $\ket{\downarrow\downarrow}, \ket{\uparrow\downarrow},$ and $\ket{\downarrow\uparrow}$,  
%$\mc{V}_{\mr{Ryd}}$.%the constrained subspace
Similarly as in Ref.~\cite{Lin2019mps} we identify them
with the states of an artificial $S=1$ {``block-spin"} by defining {$\ket{0}_b\coloneqq\ket{\downarrow\downarrow}_{b_\alpha,b_\beta}, \ket{+}_b\coloneqq\ket{\downarrow\uparrow}_{b_\alpha,b_\beta}$, and $\ket{-}_b\coloneqq\ket{\uparrow\downarrow}_{b_\alpha,b_\beta}$},
where $\ket{\pm}$ and $\ket{0}$ are eigenstates of the corresponding $S^z$-operator with eigenvalues $\pm1$ and $0$, respectively. 

%The subscript $b$ indicates a site of the block-spin, which is defined more precisely below. 

{{Let us now consider a dimerization of the lattice, i.e., a covering of all lattice sites with a  set $\Lambda_{\mr{B}}$ of disjoint bonds $b$ (see Fig.~\ref{fig:lattice}). In general this choice is not unique. }
%although in general we cannot uniquely determine a way to cover the whole lattice with such dimers 
 %A particular dimer-covering can be viewed as a lattice of dimers $\Lambda_{\mr{B}}\subset E$, where elements should cover the whole lattice, i.e., $\bigcup_{(i,j)\in\Lambda_{\mr{B}}}\{i,j\}=\Lambda$ and they are not overlapping with each other, i.e., $\{i,j\}\cap\{i',j'\}=\emptyset$ for different elements $(i,j),(i',j')\in\Lambda_{\mr{B}}$. 
 We then write $b\equiv(i,j)\in\Lambda_{\mr{B}}$, and $b_\alpha\equiv i\,(b_\beta\equiv j)$ if $i\in\Lambda_\alpha\,(j\in\Lambda_\beta)$. For any particular choice of the dimer-covering $\Lambda_{\mr{B}}$, the PXP Hamiltonian can be expressed in the} associated $S=1$ basis as 
\begin{equation}\label{eq:decomposition H}
    \begin{split}
    {H=H_{\mr{Z}}+H_1+H_2,}
    \end{split}
\end{equation}
{where}
%{MM: I think the formula for $H_1$ is not quite correct. But it is anyway too hard to read. Better express $H_1$  with the help of $1-\prod_{b_j| b_{j\alpha}\in \partial b_{\alpha}-\{ b_\beta\}} \dyad*{-}{-}_{b_j}$so that one can understand where this formula comes from.}
\begin{equation}\label{eq:pxp block-basis}
    \begin{split}
    {H_{\mr{Z}}}&{\coloneqq\sqrt{2}\sum_{b\in\Lambda_{\mr{B}}}S_b^x,}\\
    {H_1}&{\coloneqq\sum_{b\in\Lambda_{\mr{B}}}\dyad{0}{+}_b\left(\prod_{\substack{c\in\Lambda_{\mr{B}}\\c_\beta\in\partial b_\alpha\setminus\{b_\beta\}}}\left(1-\dyad*{-}\right)_c-1\right)}\\
    &{+\sum_{b\in\Lambda_{\mr{B}}}\dyad*{0}{-}_b\left(\prod_{\substack{d\in\Lambda_{\mr{B}}\\d_\alpha\in\partial b_\beta\setminus\{b_\alpha\}}}\left(1-\dyad*{+}\right)_d-1\right)}
    %\blue{H_1}&\coloneqq\blue{\sum_{b\in\Lambda_{\mr{B}}}\sum^{z_{b_\beta}-1}_{k=1}(-1)^k\dyad*{0}{+}_b\prod_{\substack{\{b_j\}_{j=1}^k\\(b_{j\alpha},b_\beta)\in E}}\dyad*{-}{-}_{b_j}}\\
    %&+\blue{\sum_{b\in\Lambda_{\mr{B}}}\sum_{k=1}^{z_{b_\alpha}-1}(-1)^k\dyad*{0}{-}_b\prod_{\substack{\{b_j\}_{j=1}^k\\(b_\alpha,b_{j\beta})\in E}}\dyad*{+}{+}_{b_j}},%\\
    %\blue{H_2}&\blue{\coloneqq-\sum_{b\in\Lambda_{\mr{B}}}\sum_{k=1}(-1)^k\dyad*{+}{0}_b\prod_{\substack{\{b_j\}_{j=1}^k\\(b_{j\alpha},b_\beta)\in E}}\dyad*{-}{-}_{b_j}}\\
    %&\blue{-\sum_{b\in\Lambda_{\mr{B}}}\sum_{k=1}(-1)^k\dyad*{-}{0}_b\prod_{\substack{\{b_j\}_{j=1}^k\\(b_\alpha,b_{j\beta})\in E}}\dyad*{+}{+}_{b_j},}
    \end{split}
\end{equation}
and $H_2=H_1^\dag$. 
%\green{Here we heve defined $\partial i\coloneqq\{j\in\Lambda|(i,j)\in E\}$.} 
We now view $H_1$ and $H_2$ as perturbations of the leading Zeeman term $H_Z$, which acts on the set of block spins of $S=1$. {Later we will find it useful to write the product over projectors as a sum over increasingly many neighbors and express $H_1$ in the following way,}
\begin{equation}\label{eq:H1 expanded}\begin{split}
    {H_1}&{=\sum_{b\in\Lambda_{\mr{B}}}\left(\sum_{k=1}^{z_{b_\alpha}-1}(-1)^kh^{k;\alpha}_b+\sum_{k=1}^{z_{b_\beta}-1}(-1)^kh^{k;\beta}_b\right)}\\
    {h^{k;\alpha}_b}&{=\sum_{\substack{\{c_j\}_{j=1}^k\subset\Lambda_{\mr{B}}\\(c_j)_\beta\in\partial b_\alpha\setminus\{b_\beta\}}}\dyad*{0,-,\cdots,-}{+,-,\cdots,-}_{b,c_1,\cdots,c_k}}\\
    {h^{k;\beta}_b}&{=\sum_{\substack{\{d_j\}_{j=1}^k\subset\Lambda_{\mr{B}}\\(d_j)_\alpha\in\partial b_\beta\setminus\{b_\alpha\}}}\dyad*{0,+,\cdots,+}{-,+,\cdots,+}_{b,d_1,\cdots,d_k},}
    \end{split}
\end{equation}
{where $z_i$ is the coordination number of the site $i$.}
{
%$z_i(i\in\Lambda)$ is the coordination number of the site $i$. 
At the level of block spins the Rydberg constraint only has to be imposed between adjacent block spins and takes the following form,} %$\blue{P_{\mr{Ryd}}=\prod_{(b_\beta,b'_\alpha)\in E}\left(1-\dyad{+,-}\right)_{b,b'}}$.}
\begin{equation}\label{eq:projector}
    {P_{\mr{Ryd}}=\prod_{(b_\beta,b'_\alpha)\in E}\left(1-\dyad*{+,-}\right)_{b,b'}.}
\end{equation}
{$P_{\mr{Ryd}}$ can now be seen as a projecting map from the spin-$1$ space $\mb{C}^{3\otimes N_b}$ to the Rydberg-constrained subspace $\mc{V}_{\mr{Ryd}}$.}

{Note that in general, a dimer covering breaks some lattice symmetries of the original model, and thus some of the symmetries of the original $S=1/2$ model cannot, {or at least not easily}, be expressed at the level of the $S=1$ representation, such that the $S=1$ Hamiltonian only possesses a reduced set of symmetries.} {We will address this issue in Sec.~\ref{sec:analytical approximation}, where we will see that the trial wavefunctions of the scar states that we will construct from specific dimerizations do not depend on that choice.} 

\subsubsection{{PXP chain}}
{For the one-dimensional PXP model with PBC, we may choose the dimer-covering $\Lambda_{\mr{B}}\coloneqq\{(2b-1,2b);\,1\leq b\leq N_b\}$. With this choice, the "perturbations" read}
\begin{equation}\begin{split}
    {H_1}&{=-\sum_{b\in\Lambda_{\mr{B}}}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{+,-}_{b,b+1}}.%\\
    %\blue{H_2}&\blue{=-\sum_{b\in\Lambda_{\mr{B}}}\ket*{+,-}\left(\bra*{+,0}+\bra*{0,-}\right)_{b,b+1}.}
    \end{split}
\end{equation}
{Note that when expressed in the block spin ($S=1$) basis, the model is only explicitly invariant with respect to translations by a full block spin or dimer, which corresponds to two $S=1/2$ sites, i.e., $T^2$. The invariance under $T$ is instead hidden in this basis.}

It is worth noting that with $H$ written in the form of Eqs.~\eqref{eq:decomposition H}{-\eqref{eq:H1 expanded}}  one can elegantly recover the  exact non-thermal zero energy eigenstate of {the 1D PXP model} that was found in Ref.~\cite{Lin2019mps}, as we show in {Appendix.}~\ref{app:ML state}. 

Numerical studies have established that the PXP chain hosts a set of ${2N_b}+1$ nonthermal eigenstates, $\ket*{\mc{S}^{\mr{PXP}}_n}$, that have high overlap with the N\'eel state $\ket{\mb{Z}_2}\coloneqq\bigotimes_{b\in\Lambda_{\mr{B}}}\ket{\downarrow\uparrow}_{{2b-1,2b}}=\bigotimes_{b\in\Lambda_{\mr{B}}}\ket{+}_b$. Moreover, these states have {almost equidistant} energies $E_n-E_{n-1}\approx \Omega_{\mr{PXP}}=1.33$ in the middle of the spectrum, while their spacing decreases towards the tails of the spectrum, (e.g. ${E_{N_b}-E_{N_b-1}}\approx0.968$ for ${N_b=10}$ block spins). %Here we do not consider zero-energy states because of huge degeneracy. However, the energies $E_n$ are not strictly equidistant: the above observation is accurate only when $n$ is small and for large $n$ the spacing tends to be smaller. For example, we numerically observe that the spacing is reduced to $E_N-E_{N-1}\approx0.968$ for $N=10$. 
However, the question as to what characterizes these scar states and how the subspace they span relates to a decomposition of the Hamiltonian as in  Eq.~\eqref{eq:pxp block-basis} has remained open.



\subsubsection{{Honeycomb lattice}}
{A natural dimer covering for the honeycomb lattice is $\Lambda_{\mr{B}}\coloneqq\{\Vec{R}\equiv(\Vec{r},\Vec{r}+\Vec{e}_y);\Vec{r}\in\Lambda_\alpha\}$. In this case, the perturbations become}
\begin{equation}\begin{split}
    H_1=&-\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\sum_{i=1,2}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{+,-}_{\Vec{R},\Vec{R}+\Vec{e}_i}\\
    &+\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\dyad*{0,-,-}{+,-,-}_{\Vec{R},\Vec{R}+\Vec{e}_1,\Vec{R}+\Vec{e}_2}\\
    &+\sum_{\Vec{R}\in\Lambda_{\mr{B}}}\dyad*{+,+,0}{+,+,-}_{\Vec{R}-\Vec{e}_1,\Vec{R}-\Vec{e}_2,\Vec{R}}.
    \end{split}
\end{equation}
By exact diagonalization of this model with PBC's (with $N_1 = N_2=3 $ unit cells in the directions $\vec{e}_{1,2}$, respectively), we found that it also hosts a similar set of $2N_b+1$ nonthermal eigenstates $\ket*{\mc{S}^{\mr{PXP}}_n}$ that have high overlap with the N\'eel state $\ket*{\mb{Z}_2}\coloneqq\bigotimes_{\Vec{r}\in\Lambda_\alpha}\ket*{\downarrow\uparrow}_{\Vec{r},\Vec{r}+\Vec{e}_y}=\bigotimes_{\Vec{R}\in\Lambda_{\mr{B}}}\ket*{+}_{\Vec{R}}$. % Like the 1D case, they have almost equidistant energies $E_n-E_{n+1}\approx$.}
Like in the 1D case, the spin-1 formulation of this model of a specific dimerization does not reflect the site-centered rotational symmetry anymore.
\begin{comment}
\subsubsection{\blue{Decorated Bethe lattice}}
\blue{By construction of the lattice $\Lambda$, we can find the dimer-covering that is isomorphic to a subset of the Bethe lattice. Each dimer can be specified by its layer $n$ and height $h$ as shown in Fig.~[FIG]. The coordinate of a dimer is then denoted by $\Vec{r}\equiv(n\,h)$. Note that the neighboring sites of $\Vec{r}$ in the $n+1$th layer are $\Vec{r}'\coloneqq(n+1\,2h+1)$ and $\Vec{r}''\coloneqq(n+1\,2h)$. The perturbations are then written as follows,} 
\begin{equation}\begin{split}
    \blue{H_1}&\blue{=-\sum_{\Vec{r}\in\Lambda_{\mr{B}}}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{+,-}_{\Vec{r},\Vec{r}'}}\\
    &\blue{-\sum_{\Vec{r}\in\Lambda_{\mr{B}}}\left(\ket*{+,0}+\ket*{0,-}\right)\bra*{+,-}_{\Vec{r},\Vec{r}''}}\\
    &\blue{+\sum_{\Vec{r}\in\Lambda_{\mr{B}}}\dyad*{0,-,-}{+,-,-}_{\Vec{r},\Vec{r}',\Vec{r}''}.}
    \end{split}
\end{equation}
\blue{This model, too, has a set of nonthermal eigenstates $\ket*{\mc{S}_n^{\mr{PXP}}}$ which have high overlap with the N\'eel state $\ket*{\mb{Z}_2}\coloneqq\bigotimes_{\Vec{r}\in\Lambda_{\mr{B}}}\ket*{+}_{\Vec{r}}$ with almost equidistant energies $E_n-E_{n-1}\approx$.}
\end{comment}

We will see {later} that neither the Zeeman term $H_{\mr{Z}}$, nor $H_1+H_2$ correspond directly to the parts $H_{\mr{spec}}$ and $H_{\mr{ann}}$ of a standard decomposition of $H$ acting on the Rydberg-constrained Hilbert space. However, the Zeeman term and the closeness of its magnitude $\sqrt{2}$ to $\Omega_{\mr{PXP}}$ 
%in Eq.~\eqref{eq:pxp block-basis} 
suggest that the relevant Hilbert space to consider is the full $S=1$ sector $\mb{C}^{3\otimes N}$ of the chain, rather than merely its smaller subspace $\mc{V}_{\mr{Ryd}}$.
Moreover, in order to establish a connection of the Rydberg system to other models with exactly known scar states, the structure found there needs to be generalized to a system with constraints. 

%\blue{We note that when $|\Lambda_\alpha|\not=|\Lambda_\beta|$, e.g., the decorated honeycomb lattice, we cannot define the lattice of dimers $\Lambda_{\mr{B}}$ as it is not possible to cover every site with dimers. However, in many cases one can cover them \textit{locally} with dimers (see Fig.~[FIG]). As we will show in the subsequent sections, our theory can apply in such a situation.}
%\begin{comment}
%\subsection{Scar states}
%\Comment{The logical flow is not clear here. You probably want to say that PXP contains {\em at least} one non-ETH eigenstate (which have been termed quantum scars in vague analogy to low energy eigenstates of quantum billiards that display non-trivial density patterns, and thus deviate from the spatial equidistribution expected in equilibrium at least at high energies). However, one should also mention the exponential degeneracy of zero energy states.
%Do people know whether there are more than 1 or 2 scar states? Maybe we can show explicitly (using the idea of solving Schroedinger's equation in the set of island states) that one can find {\em a lot} of linearly independent non-thermal eigenstates? That would be one more new thing to report.  
%}

%The PXP model is unusual in that it contains special eigenstates that violate ETH~\cite{turner_tower}.
%An explicit example of such special states has been found at energy $E=0$, i.e. in the center of the many body spectrum, in the form of a finite rank matrix product state (MPS) $\ket{\Psi_0}$ \cite{tos_aklt}, given by
%\begin{equation}\label{aklt_state}
	%\ket{\Psi_0}=\sum_{\left\{\sigma_i\right\}_{i=1}^N}\mathrm{Tr}\left[B^{\sigma_1}C^{\sigma_2}\cdots B^{\sigma_{N-1}}C^{\sigma_N}\right]\Ket{\sigma_1\cdots\sigma_N},
%\end{equation}  
%where $\sigma_i$ equals either $\uparrow$ or $\downarrow$, and $B^\sigma$ and $C^\sigma$ are matrices defined as
%\begin{equation}\begin{split}
		%B^\downarrow&=\begin{pmatrix}
			%1 & 0 & 0\\ 0 & 1 & 0
		%\end{pmatrix},\,\,
		%B^\uparrow=\sqrt{2}\begin{pmatrix}
			%0 & 0 & 0\\1 & 0 & 1
		%\end{pmatrix}\\
		%C^\downarrow&=\begin{pmatrix}
			%1 & -1\\ 1 & 0\\ 0 & 0
		%\end{pmatrix},\,\,
		%C^\uparrow=\sqrt{2}\begin{pmatrix}
			%1 & 0\\0 & 0\\-1 & 0
		%\end{pmatrix}.
	%\end{split}
%\end{equation}
%A second zero-energy "scar state" is obtained by translation by one lattice spacing. This special scar state was found
%through a mapping of the PXP model to a modification of the AKLT model \cite{original_aklt} of $S=1$ spin chains~\cite{qmbs_aklt_vp,Shiraishi_2019}, $\ket{\Psi_0}$ being the pull-back of the ground state of the latter under this mapping. The above MPS state is obviously non-thermal, as is evident from its "area-law" entanglement.

%\Comment{What should the reader do with this information?}

%\end{comment}
\begin{comment}
\textit{Known exact states for PXP model.}--In Ref.~[REF], an exact zero energy state for PBC and four eigenstates for OBC were found. They are given as matrix product states (MPS), and later a more elegant proof for the zero energy state of PBC was provided in Ref.~\cite{Shiraishi_2019}. We will re-derive those states. To do so, we introduce the following operator $A_b:\mb{C}^{2\otimes2}\rightarrow\mb{C}^3$ for $b\in\Lambda_{\mr{B}}$:
\begin{equation}\begin{split}
    A_b&\coloneqq\ket{+}_b\bra{\uparrow\uparrow}_{(b,L), (b,R)}+\frac{1}{\sqrt{2}}\ket{0}_b\left(\bra{\uparrow\downarrow}+\bra{\downarrow\uparrow}\right)_{(b,L),(b,R)}\\
    &+\ket{-}_b\bra{\downarrow\downarrow}_{(b,L),(b,R)},
    \end{split}
\end{equation}
where $(b,L/R)\in\Lambda_{\mr{B}}^{\mr{frac}}=\Lambda_{\mr{B}}\times\{L,R\}$ is a site of the ``fractional spin-$1/2$". We also define $\msf{A}\coloneqq\bigotimes_{b\in\Lambda_{\mr{B}}}A_b$. Note that for an arbitrary operator-valued function $F$, it holds that
\begin{equation}\label{eq:operator identity}
F(\bm{S}_b)\msf{A}=\msf{A}F\left(\frac{\bm{\sigma}_{(b,L)}}{2}+\frac{\bm{\sigma}_{(b,R)}}{2}\right),
\end{equation}
where $\bm{S}_b$ is a spin-$1$ operator and $\bm{\sigma}_{(b,L/R)}$ is a Pauli matrix. 

% and summarize important properties of the ground state of the AKLT model. 

%Firstly, we change the basis from the block-spin basis to the standard spin-$1$ basis, i.e., $\ket{\pm}$ and $\ket{0}$ such that $\bm{S}^2\ket{\pm}=2\ket{\pm}, \bm{S}^2\ket{0}=2\ket{0}$, $S^z\ket{\pm}=\pm\ket{\pm}$, and $S^z\ket{0}=0$ with the spin operators $\bm{S}=(S^z\,\,S^y\,\,S^z)$, according to the following prescription:
%\begin{equation}\label{eq:transformation rule}
    %\begin{cases}
    %\ket{L}_{2n}&\rightarrow\ket{+}_{2n}\\
    %\ket{R}_{2n}&\rightarrow\ket{-}_{2n}\\
    %\ket{O}_{2n}&\rightarrow\ket{0}_{2n}
    %\end{cases},
    %\begin{cases}
    %\ket{L}_{2n+1}&\rightarrow\ket{-}_{2n+1}\\
    %\ket{R}_{2n+1}&\rightarrow\ket{+}_{2n+1}\\
    %\ket{O}_{2n+1}&\rightarrow\ket{0}_{2n+1}
    %\end{cases}.
%\end{equation}
%In this spin-$1$ basis, $H_{\mr{PBC}}$ is re-written as
%\begin{equation}\label{eq:pxp PBC spin-1}\begin{split} 
    %&H_{\mr{PBC}}=\sqrt{2}\sum_{b=1}^{N/2}S_b^x\\&-\sqrt{2}\sum_{n=1}^{N/2}\big(\dyad{T_{2,2}}{T_{2,1}}+\dyad{T_{2,1}}{T_{2,2}}\big)_{2n-1,2n}\\
    %&-\sqrt{2}\sum_{n=1}^{N/2}\big(\dyad{T_{2,-2}}{T_{2,-1}}+\dyad{T_{2,-1}}{T_{2,-2}}\big)_{2n,2n+1}.
    %\end{split}
%\end{equation}

%The VBS state $\ket{\Phi_{\mr{VBS}}}$ is annihilated by any operator of a form $\dyad{T_{2,M}}{T_{2,M'}}$, and it is the unique ground state of the $SU(2)$ invariant Hamiltonian, implying it is one dimensional irreducible representation of $SU(2)$, i.e., $\sum_iS_i^x\ket{\Phi_{\mr{VBS}}}=0$. This completes the proof.
The zero energy state $\ket*{\Gamma}$ with PBC is obtained as follows
\begin{equation}
    \ket*{\Gamma}=\msf{A}\bigotimes_{b\in\Lambda_{\mr{B}}}\frac{1}{\sqrt{2}}\left(\ket*{\uparrow\uparrow}-\ket*{\downarrow\downarrow}\right)_{(b,R),(b+1,L)},
\end{equation}
up to a normalization factor.
Note that $(\ket{\uparrow\uparrow}-\ket{\downarrow\downarrow})/\sqrt{2}$ is a triplet with total $S^x$ being zero.

Four eigenstates for OBC $\ket*{\Gamma^{\tau\tau'}}$ with $\tau,\tau'=\rightarrow,\leftarrow$ are expressed as follows: \begin{equation}\begin{split}
    \ket*{\Gamma^{\tau\tau'}}\coloneqq\msf{A}&\bigotimes_{b\in\Lambda_{\mr{B}}\setminus\{N\}}\frac{1}{\sqrt{2}}\left(\ket*{\uparrow\uparrow}-\ket*{\downarrow\downarrow}\right)_{(b,R),(b+1,L)}\\&\otimes\ket{\tau}_{(1,L)}\ket{\tau'}_{(N,R)}.
\end{split}
\end{equation} 
Here we define $\ket{\rightarrow}\coloneqq(\ket{\uparrow}+\ket{\downarrow})/\sqrt{2}$ and $\ket{\leftarrow}\coloneqq(\ket{\uparrow}-\ket{\downarrow})/\sqrt{2}$.

$\ket{\Gamma}$ and $\ket*{\Gamma^{\tau\tau'}}$ are eigenstates of $H_{\mr{Z}}$. This can be easily seen by using Eq.~\eqref{eq:operator identity}. $H_{\mr{anil}1}$ and $H_{\mr{anil}2}$ annihilate these states: for $H_{\mr{anil}1}$, by the definition of the states it is straightforward to verify that $\dyad*{\psi}{+,-}_{b,b+1}\ket*{\Gamma}=\dyad*{\psi}{+,-}_{b,b+1}\ket*{\Gamma^{\tau\tau'}}=0$ for $\forall b\in\Lambda_{\mr{B}}$, $\forall\ket{\psi}\in\mb{C}^{3\otimes2}$, and for $\forall\tau,\tau'$. For $H_{\mr{anil}2}$, by making use of the fact that $H$ and $P_{\mr{Ryd}}$ commute and that $\ket*{\Gamma}$ and $\ket*{\Gamma^{\tau\tau'}}$ are eigenstates of $P_{\mr{Ryd}}$ with eigevalue $1$, we obtain
\begin{equation}\label{eq:|Gamma>}
    \begin{split}
        H\ket*{\Gamma}&=HP_{\mr{Ryd}}\ket*{\Gamma}=P_{\mr{Ryd}}H\ket*{\Gamma}=P_{\mr{Ryd}}H_{\mr{anil}2}\ket*{\Gamma}=0,
    \end{split}
\end{equation}
where the last equality holds as $P_{\mr{Ryd}}\ket{+,-}_{b,b+1}\ket{\Xi}=0$ for $\forall b\in\Lambda_{\mr{B}}$ and for any state $\ket{\Xi}$ defined on sites $\Lambda_{\mr{B}}\setminus\{b,b+1\}$. A similar relation holds for $\ket*{\Gamma^{\tau\tau'}}$ as well. 

As we will see in subsequent sections, the Zeeman term $H_{\mr{Z}}$ corresponds to $H_{\mr{spec}}$ and $H_{\mr{anil}1}$ to $H_{\mr{anil}}$ in the previous section. $H_{\mr{anil}2}$ does not have to annihilate the scar states as long as $H$ commutes with $P_{\mr{Ryd}}$ and the scar states are eigenstates of $P_{\mr{Ryd}}$ with eigenvalue $1$, as seen in Eq.~\eqref{eq:|Gamma>}. Note that for PXP model, a relevant space $\mc{V}$ is $\mb{C}^{3\otimes N}$, which is much bigger than the constrained subspace $\mc{V}_{\mr{Ryd}}$.
\end{comment}
\begin{comment}
\subsection{\label{subsec:exact eigenstates for OBC}Four exact eigenstates for the OBC}

Next we consider four exact eigenstates for OBC, which are also found in Ref.~\cite{tos_aklt} and give a simple proof that they are eigenstates. In the spin-$1$ basis, $H_{\mr{OBC}}$ is re-written as
\begin{equation}\label{eq:pxp OBC spin-1 basis}
    \begin{split}
        &H_{\mr{OBC}}=\sqrt{2}\sum_{b=1}^NS_b^x\\
        &-\sqrt{2}\sum_{n=1}^{N/2}\big(\dyad{T_{2,2}}{T_{2,1}}+\dyad{T_{2,1}}{T_{2,2}}\big)_{2n-1,2n}\\
        &-\sqrt{2}\sum_{n=1}^{N/2-1}\big(\dyad{T_{2,-2}}{T_{2,-1}}+\dyad{T_{2,-1}}{T_{2,-2}}\big)_{2n,2n+1}.
    \end{split}
\end{equation}
%Note that we do not identify $b+N$ and $b$ for OBC.
We show that the four exact eigenstates correspond to the VBS state for OBC:
\begin{equation}
    \begin{split}
        \ket*{\Phi_{\mr{VBS}}^{\sigma\sigma'}}&\equiv\left(\bigotimes_{b'=1}^N\mc{P}_{b'}\right)\ket{\sigma}_{1,\mr{L}}\bigotimes_{b=1}^{N-1}\ket*{\psi_s}_{b,b+1}\otimes\ket*{\sigma'}_{N,\mr{R}}\\
        &\equiv\left(\bigotimes_{b'=1}^N\mc{P}_{b'}\right)\ket*{\widetilde{\Phi}_{\mr{VBS}}^{\sigma\sigma'}},
    \end{split}
\end{equation}
where $\ket{\rightarrow}$ and $\ket{\leftarrow}$ are defined as  
\begin{equation}
    \ket{\rightarrow}\equiv\frac{1}{\sqrt{2}}\left(\ket{\uparrow}+\ket{\downarrow}\right),\,\,\ket{\leftarrow}\equiv\frac{1}{\sqrt{2}}\left(\ket{\uparrow}-\ket{\downarrow}\right).
\end{equation}
Note that they are eigenstates of $X$ with eigenvalues $\pm1$.

A diagrammatic representation of $\ket*{\Phi_{\mr{VBS}}^{\sigma\sigma'}}$ is depicted in Fig.[FIG]. Physically, those states correspond to four possible combinations of polarization of the edge spin-$1/2$s in $x$-direction. It is obvious that the second and the third lines of Eq.\eqref{eq:pxp OBC spin-1 basis} annihilate $\ket*{\Phi_{\mr{VBS}}^{\sigma\sigma'}}$ irrespective of $\sigma,\sigma'$. Also, we immediately see that
\begin{equation}\begin{split}
    \left(S_{b,\mr{L}}^x+S_{b+1,\mr{R}}^x\right)\ket*{\widetilde{\Phi}_{\mr{VBS}}^{\sigma\sigma'}}&=0\quad\text{for }\forall 1\leq b\leq N-1\\
    \left(S_{1,\mr{L}}^x+S_{N,\mr{R}}^x\right)\ket*{\widetilde{\Phi}_{\mr{VBS}}^{\sigma\sigma'}}&=(\varepsilon_\sigma+\varepsilon_{\sigma'})\ket*{\widetilde{\Phi}_{\mr{VBS}}^{\sigma\sigma'}},
    \end{split}
\end{equation}
where $\varepsilon_\rightarrow\equiv+1/2,\,\, \varepsilon_\leftarrow\equiv-1/2$. Therefore $\ket*{\Phi_{\mr{VBS}}^{\sigma\sigma'}}$ are exact eigenstates with energies $\sqrt{2}(\varepsilon_\sigma+\varepsilon_{\sigma'})$. 

Intuitively, the edge spin-$1/2$s in the states $\ket*{\Phi_{\mr{VBS}}^{\tau\tau'}}$ ``feel" the magnetic field in $x$-direction that is represented by the ``Zeeman" field $\sqrt{2}\sum_bS_b^x$ in $H_{\mr{OBC}}$, and according to their polarization the energies are determined.
%\subsection{\label{subsec:tos}The Tower of State}
%As in the experiment in a Rydberg atom chain~\cite{qmbs_experiment}, the PXP Hamiltonian also shows long-lasting quantum revivals, avoiding the thermalization~\cite{turner_tower} when the initial state is the N\'{e}el's order, or $\mathbb{Z}_2$ state $\ket{\mathbb{Z}_2}\equiv\ket{\uparrow\downarrow\uparrow\cdots}$. This is because the $\mathbb{Z}_2$ state has high overlaps with a set of special eigenstates which have almost equidistant eigenenergies called the tower of state, first pointed out in Ref.~\cite{Turner2018} (Fig.\ref{fig:pbc_z2overlap_n_14}). The tower of states exists not only in the PXP model, but also in other models \cite{tos_aklt, tos_xy, tos_exact_2}. %The PXP model, unlike any other models hosting the tower of states, does not have the {\it exact} tower of states, which means spectrum is only {\it approximately} equidistant. 
%Note that spectrum of the tower of states in the PXP model is not exactly equidistant, while other models are fine-tuned to have an exactly equidistant tower of states.

%\begin{figure}
	%\centering
	%\includegraphics[width=.48\textwidth]{overlap_z2_more_editted.pdf}
	%\caption{\label{fig:pbc_z2overlap_n_14}Overlap between the $\mathbb{Z}_2$ state and eigenstates for $N=20$. The red dots correspond to the tower of states. The red dot located at the center of the spectrum ($E=0$) has the highest overlap with $\mathbb{Z}_2$ state.}
%\end{figure}

%Several mechanisms have been discussed to explain the emergence of the tower of states for the PXP model, most of which leverage some algebraic structures it contains. One such example is the so-called nearly $SU(2)$ algebra: a set of non-local operators form $SU(2)$ algebra approximately \cite{nearly_su2}, which is developed to the more general notion of weakly broken lie algebra~\cite{Kieran2020}. Another example is found in Ref.~\cite{magnon_condensation}. Their strategies are essentially the same in that a certain set of (non-local) operators are almost closed in terms of commutation relations and within a certain subspace generated by those operators the tower of states are sought. %This idea is further developed so as to make algebra perfectly closed by adding perturbations [Ref].

%Here we formulate the above-mentioned idea following SGA \cite{eta_pair_rsga} and the mechanism in Ref.~\cite{tos_aklt_unified}. Firstly, we require an operator $Q^\dagger$  satisfy the following equation
%\begin{equation}\label{eq:relation}
	%\left[H, Q^\dagger\right]=\omega Q^\dagger+A.
%\end{equation}
%We do not require (anti)commutation relation for the operators $Q$ and $Q^\dagger$ and $Q^\dagger$ is non-local in general.
%Nevertheless we refer to $Q^\dagger$ as a ``creation" operator since Eq.\eqref{eq:relation} is similar to the equation of motion of the harmonic oscillator. 
                         
%We should also find a reference state $\ket{\psi}$ lying in the tower of states with an energy $E$. If $Q^\dagger$ is the creation operator which constructs the tower of state with exactly equidistant energies, $A$ must annihilate any state constructed by $Q^\dagger$ and $\ket{\psi}$. Therefore for any $n$, 
%\begin{equation}\label{exact_condition}
	%A\left(Q^\dagger\right)^n\ket{\psi}=0
%\end{equation}  
%holds. If this is the case, $\left(Q^\dagger\right)^n\ket{\psi}$ is an eigenstate with an eigenenergy $E+n\omega$. These states span a subspace $\mathcal{V}$ as
%\begin{equation}\label{subspace}
	%\mathcal{V}=\mathrm{span}\left\{\left(Q^\dagger\right)^n\ket{\psi}, 0\leq n\leq n_{\max}\right\},
%\end{equation}
%where $n_{\max}$ is some integer meaning the maximum number of excitations. Any state inside this subspace exhibits a periodic time-evolution with a frequency $\omega$ or multiples of $\omega$. 
%On the other hand, we do not expect such a structure in the PXP model since the exact tower of states does not exist. Thus we should relax the condition (Eq.\eqref{exact_condition}) and only require 
%\begin{equation}\label{eq:gamma_n}
	%\gamma_n\equiv\frac{\left\|A\left(Q^\dagger\right)^n\ket{\psi}\right\|}{\left\|\omega Q^\dagger\left(Q^\dagger\right)^n\ket{\psi}\right\|}
%\end{equation}    
%be small for $0\leq n\leq n_{\max}-1$.

%Note that the towers of states discussed in Refs.~\cite{tos_aklt, tos_exact_2,tos_xy} are explained by this formalism as special cases where Eq.\eqref{exact_condition} is satisfied. However, the tower of states in the PXP model has not been considered in this formalism although Ref.~\cite{nearly_su2}, Ref.~\cite{Kieran2020}, and Ref.~\cite{magnon_condensation} apparently satisfy the conditions (Eq.\eqref{eq:relation} and Eq.\eqref{eq:gamma_n}). In Ref.~\cite{nearly_su2} and Ref.~\cite{Kieran2020}, the reference state is $\mathbb{Z}_2$ state, which is not an eigenstate of the PXP Hamiltonian. In Ref.~\cite{magnon_condensation}, the reference state is the ground state, which does belong to the tower of states, but successive actions of the ``$\pi$ magnon" creation operator does not yield another member of the tower of states.
\end{comment}

==> summary_outlook.tex <==
The present study elucidates the structure of the anomalous eigenstates that violate the ETH in Rydberg {arrays defined on a wide class of lattices}. The original PXP model, and even more so its various scar-enhanced modifications, exhibit scar states having remarkably high overlap with the analytically given projected maximal spin states, $\ket*{S_n}$ of Eq.~\eqref{eq:trial state}. 

We further showed that the PXP model is proximate to scar-enhanced modifications which fit the universal algebraic structure governing essentially all known models hosting exact towers of scars. The usually encountered decomposition into a simple spectral (Zeeman) term and a sum of local annihilators required, however, a generalization to the case of a fragmented Hilbert space, present in the form of the Rydberg constraint in the PXP model. {This generalized structure is present independently of the lattice, as long as it is bipartite and the two sublattices have equal cardinality. We expect our ansatz for the scar wavefunctions to be close to exact scar states especially in cases where the site coordination number is low. For such cases, we can  rationalize the emergence of scar states in the PXP model. %This is illustrated by the universal structure that is approximately present in the PXP Hamiltonian, 

By leveraging the discovered structure underlying the scars, we have constructed an explicit non-Hermitian perturbation which preserves the Rydberg constraint and possesses the wavefunctions $\ket*{S_n}$ as {\em exact} scar states. Interestingly, the Hermitian part of this systematically constructed perturbation coincides with modifications that were previously studied in the literature on a more empirical basis.} 

The dynamics resulting in these systems is that of a precessing macro-pseudospin whose motion is projected onto the manifold of states obeying the Rydberg constraint. While the picture of a big spin has been suggested in previous works, we provide here an explicit construction of this spin and the associated scar wavefunctions from the elementary degrees of freedom.

Our construction makes use of an explicit dimerization of the bipartite lattice to define a spin space that extends the Rydberg-constrained manifold and breaks certain lattice symmetries. Interestingly, however, the trial scar states we obtain upon projection to the Rydberg manifold, do not depend on the choice of the dimerization, unlike their pre-images. This raises the interesting open question as to whether there might be a unique, dimerization-independent  way to define a parent spin space whose large-spin states project to the scar states.

We demonstrated the dimerization independence by casting the wavefunctions into an explicit form showing that they consist in specific superpositions of maximal spin states on the two sublattices. It will be interesting to explore this form further and establish connections with approaches that consider bipartite structures with very large connectivity~\cite{PhysRevLett.128.090606}.


%Also we considered a Hermitian perturbation which is discussed in the literature and analytically obtained its optimal coupling constant, which is in an excellent agreement with the numerics.

%We note that scar states can often be understood as a ``lift" of spin-$1/2$ states~\cite{KO2022}. One can define a suitable subspace which is isomorphic to the spin-$1/2$ Hilbert space, and the scar states, after a suitable unitary transformation, become highly symmetric states. Local annihilating terms in $H_{\mr{ann}}$ consist of projectors which project out the scar states. Interestingly, we saw that the scar states in the PXP model are \textit{not} mapped to such spin-$1/2$ states.   
In the literature, a variety of Hermitian modifications of $H_{\rm PXP}$ and iterative schemes to construct quasi-local models with exact scar states have been discussed. Even though they have often succeeded in greatly enhancing the periodic motion, it is not yet clear whether and why these schemes really converge or whether they are asymptotic in nature. It would be interesting to re-analyze those schemes within the framework and the general structure underlying scar-hosting models we have uncovered here. 

Likewise it will be interesting to apply the insights of this work to {systems with inequivalent sublattices. In the approach presented here, the formation of block spins on dimers was central. This required the two sublattices to have equal cardinality ($|\Lambda_\alpha|=|\Lambda_\beta|$). However, empirically, scar states were also found  numerically in systems with two inequivalent sublattices ($|\Lambda_\alpha|\not=|\Lambda_\beta|$), such as on the decorated honeycomb lattice. Indeed it has been shown that various two-dimensional lattices of Rydberg atoms exhibit similar quantum revivals of an initial  density-wave state, which can be further stabilized by Floquet engineering~\cite{Bluvsteineabg2530}.
} {In those cases it might be interesting to explore generalizations of the wavefunction ansatz Eq.~\eqref{eq:|Sn> inv}, which does not  rely on a dimerization.
}%higher dimensional models with constraints,such as the experimentally important Rydberg blockade.
% In particular it is an interesting open question to establish which objects play the role analogous to the block spin $S=1$ degrees of freedom in the Rydberg chain. 


